Learning Meta Face Recognition in Unseen Domains

Face recognition systems are usually faced with unseen domains in real-world applications and show unsatisfactory performance due to their poor generalization. For example, a well-trained model on webface data cannot deal with the ID vs. Spot task in surveillance scenario. In this paper, we aim to learn a generalized model that can directly handle new unseen domains without any model updating. To this end, we propose a novel face recognition method via meta-learning named Meta Face Recognition (MFR). MFR synthesizes the source/target domain shift with a meta-optimization objective, which requires the model to learn effective representations not only on synthesized source domains but also on synthesized target domains. Specifically, we build domain-shift batches through a domain-level sampling strategy and get back-propagated gradients/meta-gradients on synthesized source/target domains by optimizing multi-domain distributions. The gradients and meta-gradients are further combined to update the model to improve generalization. Besides, we propose two benchmarks for generalized face recognition evaluation. Experiments on our benchmarks validate the generalization of our method compared to several baselines and other state-of-the-arts. The proposed benchmarks will be available at https://github.com/cleardusk/MFR.

==> analysis.tex <==
\section{Analysis}
The first order Taylor expansion has the following form:
\begin{equation}
    \label{eq_taylor}
    f(x) = f(x_0) + f'(x_0) \times (x - x_0),
\end{equation}
where $x_0$ is a value close to $x$. Let $x = \theta - \alpha \mathcal{L}_S'(\theta)$ and $x_0 = \theta$, the second term of Eqn.~\ref{eq_finalobj} becomes:
\begin{equation}
    \label{eq_meta_taylor}
    \mathcal{L}_T (\theta - \alpha \mathcal{L}_S'(\theta)) = \mathcal{L}_T(\theta) + \mathcal{L}_T' (\theta) \cdot (-\alpha \mathcal{L}_S'(\theta)).
\end{equation}
Then the meta objective Eqn.~\ref{eq_finalobj} becomes:
\begin{equation}
	\argmin_\theta  \gamma \mathcal{L}_S (\theta) +  (1-\gamma) \mathcal{L}_T(\theta) - \alpha (1-\gamma)  ( \mathcal{L}_S'(\theta) \mathcal{L}_T'(\theta) ).
\end{equation}
It indicates that the model is optimized to: (i) minimize the loss on both meta-train and meta-test domains. (ii) maximize the dot product of $\mathcal{L}_S'(\theta)$ and $\mathcal{L}_T'(\theta)$. The former is obvious as we want to learn discriminative embeddings on both domains. For the latter, if we regard $\mathcal{L}_S'(\theta) \mathcal{L}_T'(\theta)$ as the similarity between two gradient vectors, it can be understood as we want to encourage two gradients on both domains towards a similar direction.
In contrast, the conventional objective $\argmin_\theta \mathcal{L}_S (\theta) + \mathcal{L}_T (\theta)$ has no such constraint.

%This explaination 

